Plottery: A Code-Integrated GUI for Matplotlib

Scientists have many tools to author plots: graphical direct manipulation apps like a spreadsheet's chart builder, text-based programming tools like Matplotlib and ggplot2, or AI chat interfaces. Textual code is the most capable of these, but writing code, even with AI assistance, is a potentially poor fit for graphical chart design. We present Plottery, a Jupyter notebook extension that leverages API type annotations to add graphical direct manipulation to the popular Matplotlib plotting library. User interactions in Plottery's in-situ graphical interface are immediately reified in the user's code, so they may seamlessly mix-and-match between GUI, code, and AI interactions. In a user study, participants seamlessly alternated modalities, with the GUI used for straightforward visual changes, code for quick edits or duplicating code, and the AI for broad support. Plottery showcases graphical interaction that retains code's benefits.

==> acknowledgements.tex <==
\section*{Acknowledgments}

\todo{Thanks to William Duan for crucial aid in the initial setup of NPM and TypeScript,
to Matthew Beaudouin-Lafon for insightful comments on the limitations of the user study,
and to Damien Masson for insightful discussions about other ways \sys could have been designed.
This work was supported by U.S. National Science Foundation Grants No. 2432644 (\emph{Direct Manipulation for Everyday Programming}) and No. 2107397 (\emph{Human-Centric Program Synthesis}).
}

